The Effects of Adding Reachability Predicates in Quantifier-Free Separation Logic

The list segment predicate ls used in separation logic for verifying programs with pointers is well-suited to express properties on singly-linked lists. We study the effects of adding ls to the full quantifier-free separation logic with the separating conjunction and implication, which is motivated by the recent design of new fragments in which all these ingredients are used indifferently and verification tools start to handle the magic wand connective. This is a very natural extension that has not been studied so far. We show that the restriction without the separating implication can be solved in polynomial space by using an appropriate abstraction for memory states whereas the full extension is shown undecidable by reduction from first-order separation logic. Many variants of the logic and fragments are also investigated from the computational point of view when ls is added, providing numerous results about adding reachability predicates to quantifier-free separation logic.

==> proof-corollary-undecidability-limited-reach.tex <==
\begin{proof} Given a formula $\aformula$ in $\foseplogic{\magicwand}$, its translation $\mathcal{T}_{\rm SAT}(\aformula)$
in $\seplogic{\separate, \magicwand, \ls}$ uses $\ls$ in formulae of the form
$\aformula_{=}(\avariable,\avariablebis)$,
$\aformula_{\hpto}(\avariable,\avariablebis, \avariableter)$
and $\mathtt{alloc}_{\avariablebis}^{-1}(\avariable)$.
Below, we explain why in the context of the translation $\mathcal{T}_{\rm SAT}(\aformula)$, occurrences of $\reach(\avariable,\avariable')$ can be
replaced by a disjunction made of disjuncts from $\avariable = \avariable'$, $\avariable \hpto \avariable'$, $\reach(\avariable,\avariable') = 2$
or $\reach(\avariable,\avariable') = 3$.
The first property that we can use is that given a formula $\aformulabis$,
$[\aformulabis]_3$ is logically equivalent to $[\aformulabis']_3$ where $\aformulabis'$ is obtained
from  $\aformulabis$ by replacing every occurrence of $\reach(\avariable,\avariable')$ not in the scope
of a separating connective by
$
\avariable = \avariable' \vee \avariable \hpto \avariable' \vee \reach(\avariable,\avariable') = 2 \vee
\reach(\avariable,\avariable') = 3.
$
A similar property holds with $[\aformulabis]_2$ or $[\aformulabis]_1$ by removing the adequate disjuncts.
Below, we push a bit further this property and consider variants.

Let us recall below the definition the formula $\mathtt{alloc}_{\avariablebis}^{-1}(\avariable)$:
$$
\avariable \hpto \avariable \vee \avariablebis \hpto \avariable \vee
[\neg \alloc{\avariablebis} \wedge (\alloc{\avariablebis} \land \lnot \avariablebis \hpto \avariable \land \size = 1 ) \lollipop \reach(\avariablebis,\avariable)]_1
$$
It is easy to show that $\mathtt{alloc}_{\avariablebis}^{-1}(\avariable)$ is logically equivalent to
$$
\avariable \hpto \avariable \vee \avariablebis \hpto \avariable \vee
[\neg \alloc{\avariablebis} \wedge (\alloc{\avariablebis} \land \lnot \avariablebis \hpto \avariable \land \size = 1 ) \lollipop \reach(\avariablebis,\avariable) = 2]_1
$$

Similarly, let us recall below the definition of the formula $\aformula_{=}(\avariable,\avariablebis)$:
\begin{gather*}
(\avariable = \avariablebis \land \alloc{\avariable}) \lor
(\avariable \neq \avariablebis \wedge \avariable \hpto \avariablebis \land \avariablebis \hpto \avariablebis)
\lor (\avariable \neq \avariablebis \land \avariablebis \hpto \avariable \land \avariable \hpto \avariable)\lor\\
[\new(\avariable,\avariablebis) \land (\true \sepimp \lnot(\reach(\avariable,\avariablebis) \land \reach(\avariablebis,\avariable))]_2
\end{gather*}
One can show that for all memory states $\pair{\astore}{\aheap}$ with $\card{\domain{\aheap}} = 2$ and $\pair{\astore}{\aheap} \models \new(\avariable,\avariablebis)$,
we have $\pair{\astore}{\aheap} \models \true \sepimp \lnot(\reach(\avariable,\avariablebis) \land \reach(\avariablebis,\avariable))$
iff $\pair{\astore}{\aheap} \models \true \sepimp \lnot(\reach(\avariable,\avariablebis) = 2 \land
\reach(\avariablebis,\avariable) = 2)$. So, in the formula  $\aformula_{=}(\avariable,\avariablebis)$, we can safely replace
$\reach(\avariable,\avariablebis) \land \reach(\avariablebis,\avariable)$ by $\reach(\avariable,\avariablebis) = 2 \land
\reach(\avariablebis,\avariable) = 2$ in order to obtain an equivalent formula.

Finally, let us recall below the definition of the formula $\aformula_{\hpto}(\avariable,\avariablebis,\avariableter)$:

$$
[
n(\avariable) = n(\avariablebis) \Rightarrow
$$
$$
(\avariable \hpto \avariablebis \land \avariablebis \hpto \avariablebis) \lor
(\avariablebis \hpto \avariable \land \avariable \hpto \avariable) \lor [\alloc{\avariable} \land (\true \sepimp \lnot \boxed{\reach(\avariable,\avariableter)})]_2)
]
$$
$$ \wedge $$
$$
(
\neg (n(\avariable) = n(\avariablebis)) \Rightarrow
$$
$$
(\avariable \hpto \avariablebis \land \avariablebis \hpto \avariable) \lor [\avariablebis \hpto \avariablebis \land \avariable \not \hpto \avariablebis \land
\boxed{\reach(\avariable,\avariablebis)}]_3 \lor
$$
$$
[\new(\avariable,\avariablebis) \land \lnot \boxed{\reach(\avariable,\avariablebis)} \land \lnot \boxed{\reach(\avariablebis,\avariable)}
    \land
$$
$$
((\size = 1 \land \mathtt{alloc}_{\avariable}^{-1}(\avariablebis)) \lollipop \reach(\avariable,\avariablebis) = 3)\\
    \land (\true \sepimp \lnot(\boxed{\boxed{\reach(\avariable,\avariablebis)}} \land \boxed{\boxed{\reach(\avariablebis,\avariable)}}))]_3)])
$$

An equivalent formula can be obtained by replacing:
\begin{itemize}
\itemsep 0 cm
\item $\boxed{\reach(\avariable,\avariableter)}$ by $\reach(\avariable,\avariableter) = 2$ (we also use the fact that in the third disjunct
of $\aformulabis_{=}$ we can add that $\avariable \neq \avariablebis$),
\item $\boxed{\reach(\avariable,\avariablebis)}$ and $\boxed{\reach(\avariablebis,\avariable)}$ are not in the scope of a separating connective
in $[\cdot]_3$, so we can apply the substitution discussed a bit earlier,
\item $\boxed{\boxed{\reach(\avariable,\avariablebis)}}$ by $\reach(\avariable,\avariablebis) = 3$,
\item $\boxed{\boxed{\reach(\avariablebis,\avariable)}}$ by $\reach(\avariable,\avariablebis) = 2$.\qed
\end{itemize}
\end{proof}


==> proof-lemma-correctness-translation-old.tex <==
\begin{proof}
%% \SDnote{Improve the readability, add numbered labels, number equations.}
  The proof is by induction on the structure of $\aformulabis$. We start by proving the two base cases
with the atomic formulae $\avariable_i = \avariable_j$ and $\avariable_i \hpto \avariable_j$.
\begin{enumerate}
  \item Let $\aformulabis$ be $\avariable_i = \avariable_j$. We have $\{\avariable_i,\avariable_j\} \subseteq \asetbis \subseteq \aset$
  and $\atranslation(\aformulabis,\aset) = n(\avariable_i) = n(\avariable_j)$ by definition. The following equivalences hold.
  \begin{itemize}
  \item By definition of $\models$, $\pair{\astore_1}{\aheap_1} \models \avariable_i = \avariable_j$ if and only if
  $\astore_1(\avariable_i) = \astore_1(\avariable_j)$.
  \item From the third condition in Definition~\ref{def:rhd}, $\astore_1(\avariable_i) = \astore_1(\avariable_j)$ if and only if
   $$\aheap_2(\astore_2(\avariable_i)) = \aheap_2(\astore_2(\avariable_j)).$$
  \item Lastly, by definition of $\models$, $\aheap_2(\astore_2(\avariable_i)) = \aheap_2(\astore_2(\avariable_j))$ if and only if $\pair{\astore_2}{\aheap_2} \models n(\avariable_i) = n(\avariable_j)$.
  \end{itemize}
  \item Let $\aformulabis$ be
   $(\avariable_i \hpto \avariable_j)$.  We have $\{\avariable_i,\avariable_j\} \subseteq \asetbis \subseteq \aset$ and
 $\atranslation(\aformulabis,\aset) = n(\avariable_i) \hpto n(\avariable_j)$ by definition. The following equivalences hold.
  \begin{itemize}
  \item By definition, $\pair{\astore_1}{\aheap_1} \models \avariable_i \hpto \avariable_j$ if and only if $\aheap_1(\astore_1(\avariable_i)) = \astore_1(\avariable_j)$.
  \item From the third condition in the definition of $\rhd_q^{\asetbis}$,
        we have $\aheap_1(\astore_1(\avariable_i)) = \astore_1(\avariable_j)$ if and only if $\aheap_2(\aheap_2(\astore_2(\avariable_i))) = \aheap_2(\astore_2(\avariable_j))$.
  Indeed, since $\astore_1(\avariable_i) = \aheap_2(\astore_2(\avariable_i)) \in \LOC_1$ and for all $\alocation \in \LOC_1$ $\aheap_1(\alocation) = \aheap_2(\alocation)$, it holds that $\aheap_1(\aheap_2(\astore_2(\avariable_i))) = \aheap_2(\aheap_2(\astore_2(\avariable_i)))$.
  \item Lastly, by definition of $\models$, $\aheap_2(\aheap_2(\astore_2(\avariable_i))) = \aheap_2(\astore_2(\avariable_j))$ if and only if $\pair{\astore_2}{\aheap_2} \models n(\avariable_i) \hpto n(\avariable_j)$.
  \end{itemize}
  \end{enumerate}
  We now consider the induction step and we distinguish the different cases depending on the outermost connective.
  In order to be precise, we assume that the induction hypothesis is the following:
%%  (the obvious one):
  given  $\asetbis \subseteq \{\avariable_1, \ldots, \avariable_q\}$,
 $\triple{\LOC_1}{\astore_1}{\aheap_1} \rhd_q^{\asetbis} \ \triple{\LOC_2}{\astore_2}{\aheap_2}$ and a formula $\aformulabis$
  in $\foseplogic{\magicwand}$ of size $\leq N$ and with free variables among $\asetbis$,  and
$\asetbis$ does not contain any bound variable of $\aformulabis$, we have
$\pair{\astore_1}{\aheap_1}  \models \aformulabis$ iff $\pair{\astore_2}{\aheap_2} \models \atranslation(\aformulabis,\aset)$.
  In the induction step, we take a formula $\aformulabis$ of size $N+1$.

  Before treating the different cases, let us introduce the binary relation
  $\brhd^{\asetbis}_q$ defined as a slight variant of $\rhd^{\asetbis}_q$ (just the last condition is
  modified as well as the set of indices for the variables in $\asetbis$).
  So, given $\asetbis \subseteq \set{\avariable_{q+1},\dots,\avariable_{2q}}$ (the variable indices are different)
  and  two generalised memory states $\triple{\LOC_1}{\astore_1}{\aheap_1}$ and  $\triple{\LOC_2}{\astore_2}{\aheap_2}$, we write  $\triple{\LOC_1}{\astore_1}{\aheap_1} \brhd_q^{\asetbis} \ \triple{\LOC_2}{\astore_2}{\aheap_2}$
 when the  conditions below are satisfied:
\begin{enumerate}
\item $\LOC_1 = \LOC_2 \setminus \set{\astore_2(\avariable) \ \mid \ \avariable \in \aset}$,
\item for all $\avariable \neq \avariablebis \in \aset$, $\astore_2(\avariable) \not= \astore_2(\avariablebis)$,
\item $\aheap_2 = \aheap_1 + \{\astore_2(\avariable) \pto \astore_1(\overline{\avariable}) \mid \avariable \in \asetbis \}$.
\end{enumerate}
In the encoding of $\astore_1$, the variables in $\set{\avariable_{q+1},\dots,\avariable_{2q}}$ 
involved in $\brhd_q^{\asetbis}$ play the same role as the variables in $\set{\avariable_{1},\dots,\avariable_{q}}$
involved in   $\rhd^{\asetbis}_q$.

Given a set of variables $\asetter \subseteq \set{\avariable_{1},\dots,\avariable_{q}}$,
let $\overline{\asetter} \egdef \set{\overline{\avariablebis} \ \mid \ \avariablebis \in \asetter}$. One can show that
the properties below are equivalent:
\begin{itemize}
\item $\triple{\LOC_1}{\astore_1}{\aheap_1} \rhd^{\asetter}_q \triple{\LOC_2}{\astore_2}{\aheap_1 +
      \{\astore_2(\avariablebis) \pto \astore_1(\avariablebis) \mid \avariablebis \in \asetter\}}$,
\item $\triple{\LOC_1}{\astore_1}{\aheap_1} \brhd^{\overline{\asetter}}_q \triple{\LOC_2}{\astore_2}{\aheap_1 +
    \{\astore_2(\overline{\avariablebis}) \pto \astore_1(\avariablebis) \mid \avariablebis \in \asetter\}}$.
\end{itemize}
Moreover, it is easy to show that if
$\triple{\LOC_1}{\astore_1}{\aheap_1} \rhd^{\asetter}_q \triple{\LOC_2}{\astore_2}{\aheap_2}$, or alternatively
$\triple{\LOC_1}{\astore_1}{\aheap_1} \brhd^{\overline{\asetter}}_q \triple{\LOC_2}{\astore_2}{\aheap_2}$, then from the three 
conditions of their definition, it holds that
$\pair{\astore_2}{\aheap_2} \models \OK(X)$ and for all $\avariable \in (\aset \setminus \overline{\asetter})$, 
we have $\astore_2(\avariable) \not\in \domain{\aheap_2}$.

Let us write $\aheap_2 = \aheap_1 +
      \{\astore_2(\avariablebis) \pto \astore_1(\avariablebis) \mid \avariablebis \in \asetter\}$
and $\aheap^{\star}_2 = \aheap_1 +
    \{\astore_2(\overline{\avariablebis}) \pto \astore_1(\avariablebis) \mid \avariablebis \in \asetter\}$.
Now, we can equivalently reformulate the induction hypothesis as follows:
%% By the induction hypothesis, we can conclude that:
given  $\asetter \subseteq \{\avariable_{q+1}, \ldots, \avariable_{2q}\}$,
 $\triple{\LOC_1}{\astore_1}{\aheap_1} \brhd_q^{\asetter} \ \triple{\LOC_2}{\astore_2}{\aheap_2^{\star}}$ and a formula $\aformulabis$
  in $\foseplogic{\magicwand}$ with free variables among $\overline{\asetter}$ of size $\leq N$,  and
$\overline{\asetter}$ does not contain any bound variable of $\aformulabis$, we have
$\pair{\astore_2}{\aheap_2} \models \atranslation(\aformulabis,\aset)$ iff
$\pair{\astore_2}{\aheap_2^{\star}} \models \atranslation(\aformulabis,\aset)[\avariable \gets \overline{\avariable}]$
(therefore both equivalent to $\pair{\astore_1}{\aheap_1}  \models \aformulabis$).
Actually, the above property is equivalent to the induction hypothesis.

Let us start the induction step now. We omit the obvious cases for the
Boolean connectives. 
%% SD 19/05/2019
%% Obvious cases. 
%%
\cut{
The proofs for negation and conjunction are  straightforward as the translation is homomorphic for Boolean connectives.
  \begin{enumerate}
    \setcounter{enumi}{2}
    \item Let $\aformulabis = \lnot \aformula$. So $\aformula$ and $\aformulabis$ share the same set of free variables. We can therefore apply the
    induction hypothesis as shown below:
    \begin{align*}
      &\pair{\astore_1}{\aheap_1} \models \lnot \aformula
      \equivbydef \pair{\astore_1}{\aheap_1} \not\models \aformula
      \stackrel{\mbox{\begin{tiny}ind.hyp.\end{tiny}}}{\equivaut} \pair{\astore_2}{\aheap_2} \not\models \atranslation(\aformula,\aset)\\
      &\equivbydef \pair{\astore_2}{\aheap_2} \models \lnot \atranslation(\aformula,\aset)
      \equivbydef \pair{\astore_2}{\aheap_2} \models \atranslation(\lnot\aformula,\aset).
    \end{align*}
    \item Let $\aformulabis = \aformula_1 \land \aformula_2$. It holds that the free variables of $\aformula_1$ or $\aformula_2$
     are a subset of the free variables of $\aformula_1 \land \aformula_2$. We can therefore apply the induction hypothesis as shown below:
    \begin{align*}
      &\pair{\astore_1}{\aheap_1} \models \aformula_1 \land \aformula_2
      \equivbydef \pair{\astore_1}{\aheap_1} \models \aformula_1 \ \text{and} \ \pair{\astore_1}{\aheap_1} \models \aformula_2\\
      &\stackrel{\mbox{\begin{tiny}ind.hyp.\end{tiny}}}{\equivaut} \pair{\astore_2}{\aheap_2} \models \atranslation(\aformula_1,\aset) \text{ and } \pair{\astore_2}{\aheap_2} \models \atranslation(\aformula_2,\aset)\\
      &\equivbydef \pair{\astore_2}{\aheap_2} \models \atranslation(\aformula_1,\aset) \land \atranslation(\aformula_2,\aset)
      \equivbydef \pair{\astore_2}{\aheap_2} \models \atranslation(\aformula_1 \land \aformula_2,\aset)
    \end{align*}
  \end{enumerate}
}
  We now prove the result for $\forall \avariable_i \ \aformula$ and $\aformula_1 \magicwand \aformula_2$.
  \begin{enumerate}
    \setcounter{enumi}{2}
    \item Let $\aformulabis = \forall \ \avariable_i \ \aformula$ with $\avariable_i \not \in \asetbis$ and therefore by definition
    \[
      \atranslation(\forall \ \avariable_i \ \aformula,\aset) = (\alloc{\avariable_i} \wedge \size = 1) \magicwand (\Safe(\aset) \Rightarrow \atranslation(\aformula, \aset)).
    \]
    %% Moreover notice that $x_i \not\in \asetbis$ since $x_i$ is not a free variable and,
    By definition, $\pair{\astore_1}{\aheap_1} \models \forall \avariable_i \ \aformula$ if and only if for all locations $\alocation \in \LOC_1$,
    $\pair{\astore_1[\avariable_i \gets \alocation]}{\aheap_1} \models \aformula$.

    Let us now consider the generalised memory state $\triple{\LOC_2}{\astore_2}{\aheap_2 + \{\astore_2(\avariable_i) \pto \alocation\}}$.
    Since $\avariable_i \not\in \asetbis$, the heap $\aheap_2 + \{\astore_2(\avariable_i) \pto \alocation\}$ is well-defined.
    Moreover, it holds that
    \[
      \triple{\LOC_1}{\astore_1[\avariable_i \gets \alocation]}{\aheap_1} \rhd_q^{\asetbis \cup \{\avariable_i\}} \ \triple{\LOC_2}{\astore_2}{\aheap_2+ \{\astore_2(\avariable_i) \pto \alocation\}}.
    \]
    Indeed, since $\triple{\LOC_1}{\astore_1}{\aheap_1} \rhd_q^{\asetbis} \ \triple{\LOC_2}{\astore_2}{\aheap_2}$, all the conditions of
    $\rhd_q^{\asetbis \cup \{\avariable_i\}}$ are satisfied.
    By application of the induction hypothesis, we get that for all  $\alocation \in \LOC_1$, we have
    $\pair{\astore_1[\avariable_i \gets \alocation]}{\aheap_1} \models \aformula$ holds if and only if
    for all $\alocation \in \LOC_1$, $\pair{\astore_2}{\aheap_2 + \{\astore_2(\avariable_i) \pto \alocation\}} \models \atranslation(\aformula,\aset)$
    also holds.
    Moreover, due to the fulfilment of the conditions in $\rhd_q^{\asetbis \cup \{\avariable_i\}}$, any memory state $\pair{\astore_2}{\aheap_2 + \{\astore_2(\avariable_i) \pto \alocation'\}}$ satisfies
    $\Safe(\aset)$ if and only if $\alocation' \in \LOC_1$.
    Therefore, it also holds that for all $\alocation \in \LOC_1$, we have
    $\pair{\astore_2}{\aheap_2 + \{\astore_2(\avariable_i) \pto \alocation\}} \models
    \atranslation(\aformula,\aset)$ if and only if
    \[{\rm for \ all} \  \alocation \in \LOC_2,\ \pair{\astore_2}{\aheap_2 + \{\astore_2(\avariable_i) \pto \alocation\}} \models \Safe(\aset) \Rightarrow \atranslation(\aformula,\aset).\]
    Indeed, if $\alocation \in \LOC_1$ then $\Safe(\aset)$ and $\atranslation(\aformula,\aset)$ are both satisfied (for $\Safe(\aset)$, remember that all locations in $\set{\astore_2(\avariablebis) \ \mid \ \avariablebis \in \aset} \cap \domain{\aheap_2}$ already point to elements of $\LOC_1$, due to the fulfilment of the conditions in $\rhd_q^{\asetbis}$),
    otherwise whenever $\alocation \in \LOC_2 \setminus \LOC_1$ the premise of the implication  does not hold
    and therefore the formula is trivially satisfied. Observe that $\pair{\astore_2}{\{\astore_2(\avariable_i) \pto \alocation\}}$
    satisfies $\alloc{\avariable_i} \wedge \size = 1$. Then, the last formula can be written as:
    \begin{align*}
      {\rm for \ all} \ \alocation \in \LOC_2,\ &\pair{\astore_2}{\{\astore_2(\avariable_i) \pto \alocation\}} \models \alloc{\avariable_i} \wedge \size = 1\\
      \text{ implies }&\pair{\astore_2}{\aheap_2 + \{\astore_2(\avariable_i) \pto \alocation\}} \models \Safe(\aset) \Rightarrow \atranslation(\aformula,\aset),
    \end{align*}
    which is true if and only if
    \begin{align*}
      \text{for \ all \ }  \aheap', \text{ if } & (\aheap' \bot \aheap_2 \text{ and }\pair{\astore_2}{\aheap'} \models \alloc{\avariable_i} \wedge \size = 1)\\
      \text{ then }&\pair{\astore_2}{\aheap_2 + \aheap'} \models \Safe(\aset) \Rightarrow \atranslation(\aformula,\aset).
    \end{align*}
    By definition of $\models$, this is equivalent to
    \[\pair{\astore_2}{\aheap_2} \models (\alloc{\avariable_i} \wedge \size = 1) \magicwand (\Safe(\aset) \Rightarrow \atranslation(\aformula,\aset)).\]
  \item Let $\aformulabis = \aformula_1 \magicwand \aformula_2$.
  If $\pair{\astore_1}{\aheap_1} \models \aformula_1 \magicwand \aformula_2$, then by definition,
  for all heaps $\aheap_1'$, if $\aheap_1' \bot \aheap_1$ and $\pair{\astore_1}{\aheap_1'} \models \aformula_1$, then 
  we have $\pair{\astore_1}{\aheap_1+\aheap_1'} \models \aformula_2$.
  Let us show how to prove $\pair{\astore_2}{\aheap_2} \models \atranslation(\aformula_1 \magicwand \aformula_2, \aset)$.
  By definition of  $\atranslation(\aformula_1 \magicwand \aformula_2, \aset)$,
  this holds whenever for all heaps $\aheap_2'$, if $\aheap_2' \bot \aheap_2$, $\pair{\astore_2}{\aheap_2'}$ satisfies
  \[(\bigwedge_{\mathclap{\avariableter \in Z}} \alloc{\overline{\avariableter}}) \wedge
  (\bigwedge_{\mathclap{\avariableter \in \aset \setminus Z}} \neg \alloc{\overline{\avariableter}})
  \wedge \Safe(\aset) \wedge \atranslation(\aformula_1,\aset)[\avariableter \leftarrow \overline{\avariableter}]
  \]
  and $\pair{\astore_2}{\aheap_2 + \aheap_2'}$ satisfies
  $(\bigwedge_{\avariableter \in Z} n(\avariableter) = n(\overline{\avariableter})) \wedge \Safe(\aset)$,
  then $\pair{\astore_2}{\aheap_2 + \aheap_2'}$ satisfies
  \[(\bigwedge_{\mathclap{\avariableter \in \asetter}} \alloc{\overline{\avariableter}} \wedge \size = \card{\asetter}) \separate
  \atranslation(\aformula_2, \aset),\]
  where $\asetter$ is the set of free variables in $\aformula_1$.

  Let $\aheap_2'$ be some heap that satisfies the premises of the implication.
  Since $\pair{\astore_2}{\aheap_2 + \aheap_2'}$ satisfies
   $(\bigwedge_{\avariableter \in \asetter} n(\avariableter) = n(\overline{\avariableter}))$ and
   $\triple{\LOC_1}{\astore_1}{\aheap_1} \rhd_q^{\asetbis} \ \triple{\LOC_2}{\astore_2}{\aheap_2}$, which implies that
  for all $\avariablebis \in \asetbis
   \supseteq \asetter$, we have
  $\aheap_2(\astore_2(\avariablebis)) = \astore_1(\avariablebis)$, we can conclude that  for all $\avariableter \in \asetter$,
  we have $\aheap_2'(\astore_2(\overline{\avariableter})) = \astore_1(\avariableter)$. Moreover,
  $$\pair{\astore_2}{\aheap_2'} \models (\bigwedge_{\mathclap{\avariableter \in \asetter}} \alloc{\overline{\avariableter}}) \wedge
  (\bigwedge_{\mathclap{\avariableter \in \aset \setminus \asetter}} \neg \alloc{\overline{\avariableter}})
  \wedge \Safe(\aset).$$
  This entails that $\aheap_2'$ can be written as $\aheap_{\asetter} + \aheap'_1$
  where $\aheap_{\asetter} \egdef \{ \astore_2(\overline{\avariableter}) \pto \astore_1(\avariableter) \mid \avariableter
  \in \asetter \}$
  ($\aheap'_1$ is then defined as the unique subheap satisfying $\aheap_2' = \aheap_{\asetter} + \aheap'_1$,
  once $\aheap_{\asetter}$ is defined).
  Observe that the domain of $\aheap_{\asetter}$ is included in $\LOC_2$ and its codomain is 
  included in $\LOC_1$, whereas the domain $\aheap'_1$ and its codomain are included in $\LOC_1$.
  Therefore, it holds that
  \[
  \triple{\LOC_1}{\astore_1}{\aheap_1'} \brhd_q^{\overline{\asetter}}
  \triple{\LOC_2}{\astore_2}{\aheap_2'}.
  \]
  Since $\asetter$ is the set of free variables in $\aformula_1$ and
   $\pair{\astore_2}{\aheap_2'} \models \atranslation(\aformula_1,\aset)[\avariableter \gets \overline{\avariableter}]$,
  by the induction hypothesis it holds that $\pair{\astore_1}{\aheap_1'} \models \aformula_1$.
  Moreover, since $\aheap_1' \sqsubseteq \aheap_2'$,
  $\aheap_1 \sqsubseteq \aheap_2$, $\aheap_2' \bot \aheap_2$, the property $\aheap_1' \bot \aheap_1$ holds and 
  therefore, by the assumption
  $\pair{\astore_1}{\aheap_1} \models \aformula_1 \magicwand \aformula_2$,
  we also get $\pair{\astore_1}{\aheap_1 + \aheap_1'} \models \aformula_2$.
  As such, since $\triple{\LOC_1}{\astore_1}{\aheap_1 + \aheap_1'} \rhd_q^{\asetbis} \triple{\LOC_2}{\astore_2}{\aheap_2 + \aheap_1'}$
  holds because $\aheap_1'$ has domain and codomain included in $\LOC_1$ and is a subset of $\aheap_2'$ which is disjoint from $\aheap_2$,
  we can use the induction hypothesis and obtain that $\pair{\astore_2}{\aheap_2 + \aheap_1'} \models \atranslation(\aformula_2,\aset)$.

  It remains to establish that
  \[\pair{\astore_2}{\aheap_2 + \aheap_2'} \models (\bigwedge_{\mathclap{\avariableter \in \asetter}} \alloc{\overline{\avariableter}} \wedge
   \size = \card{\asetter}) \separate
  \atranslation(\aformula_2, \aset).
  \]
  Indeed, $\aheap_2' = \aheap_1' + \aheap_{\asetter}$ and
  $\pair{\astore_2}{\aheap_{\asetter}} \models \bigwedge_{\avariableter \in \asetter} \alloc{\overline{\avariableter}} \wedge
  \size = \card{\asetter}$. Lastly, as already discussed,
   $\pair{\astore_2}{\aheap_2 + \aheap_1'} \models \atranslation(\aformula_2,\aset)$.

  For the other direction, suppose that $\pair{\astore_2}{\aheap_2} \models \atranslation(\aformula_1 \magicwand \aformula_2, \aset)$.
  This means that for all heaps $\aheap_2'$ if $\aheap_2' \bot \aheap_2$, $\pair{\astore_2}{\aheap_2'}$ satisfies
  \[(\bigwedge_{\avariableter \in \asetter} \alloc{\overline{\avariableter}}) \wedge
  (\bigwedge_{\mathclap{\avariableter \in \aset \setminus \asetter}} \neg \alloc{\overline{\avariableter}})
  \wedge \Safe(\aset) \wedge \atranslation(\aformula_1,\aset)[\avariableter \leftarrow \overline{\avariableter}]
  \]
  and $\pair{\astore_2}{\aheap_2 + \aheap_2'} \models (\bigwedge_{\avariableter \in \asetter}
   n(\avariableter) = n(\overline{\avariableter})) \wedge \Safe(\aset)$,
  then
  \[\pair{\astore_2}{\aheap_2 + \aheap_2'} \models (\bigwedge_{\mathclap{\avariableter \in \asetter}}
  \alloc{\overline{\avariableter}} \wedge \size = \card{\asetter}) \separate
  \atranslation(\aformula_2, \aset),\]
  where $\asetter$ is the set of free variables in $\aformula_1$.

  Let us show how to prove that
  $\pair{\astore_1}{\aheap_1} \models \aformula_1 \magicwand \aformula_2$, which by definition holds whenever for all heaps
  $\aheap_1'$, if $\aheap_1' \bot \aheap_1$ and $\pair{\astore_1}{\aheap_1'} \models \aformula_1$ then
  $\pair{\astore_1}{\aheap_1+\aheap_1'} \models \aformula_2$.
  Let $\aheap_1'$ be a heap disjoint from $\aheap_1$ satisfying $\pair{\astore_1}{\aheap_1'} \models \aformula_1$.
  By definition of $\rhd^{\asetter}_q$,  
  \[
    \triple{\LOC_1}{\astore_1}{\aheap_1'} \rhd^{\asetter}_q \triple{\LOC_2}{\astore_2}{\aheap_1' +
    \{\astore_2(\avariableter) \pto \astore_1(\avariableter) \mid \avariableter \in \asetter\}}
  \]
  or equivalently
  \[
    \triple{\LOC_1}{\astore_1}{\aheap_1'} \brhd^{\overline{\asetter}}_q \triple{\LOC_2}{\astore_2}{\aheap_1' +
    \{\astore_2(\overline{\avariableter}) \pto \astore_1(\avariableter) \mid \avariableter \in \asetter\}},
  \]
   where $\overline{\asetter} = \set{\overline{\avariableter} \ \mid \ \avariableter \in \asetter}$.
  Let $\aheap_2' \egdef \aheap_1' + \{\astore_2(\overline{\avariableter}) \pto \astore_1(\avariableter) \mid
  \avariableter \in \asetter\}$.
  From the definition of $\brhd^{\overline{\asetter}}_q$, it holds that $\pair{\astore_2}{\aheap_2'}$ satisfies
  \[
  (\bigwedge_{\mathclap{\avariableter \in \asetter}} \alloc{\overline{\avariableter}}) \wedge
  (\bigwedge_{\mathclap{\avariableter \in \aset \setminus \asetter}} \neg \alloc{\overline{\avariableter}})
  \wedge \Safe(\aset).
  \]
  Moreover, by the induction hypothesis, we get
  $\pair{\astore_2}{\aheap_2'} \models \atranslation(\aformula_1,\aset)[\avariableter  \gets \overline{\avariableter}]$.
  Besides this, $\aheap_2$ can be written as
  $\aheap_1 + \{ \astore_2(\avariablebis) \pto \astore_1(\avariablebis) \mid \avariablebis \in \asetter\}$ 
  (condition (3) in the definition of  $\rhd_q^{\asetter}$).
  Consequently, the heap $\aheap_2 + \aheap_2'$ can be written as
  \[
    \aheap_1 + \aheap_1' + \{ \astore_2(\avariablebis) \pto \astore_1(\avariablebis) \mid \avariablebis \in \asetter\} +
   \{\astore_2(\overline{\avariableter}) \pto \astore_1(\avariableter) \mid \avariableter \in \asetter\}.
  \]
  Therefore, it holds that for all $\avariableter \in \asetter$,
  $(\aheap_2 + \aheap_2')(\astore_2(\avariableter)) = (\aheap_2 + \aheap_2')(\astore_2(\overline{\avariableter}))$ or,
  equivalently, $\pair{\astore_2}{\aheap_2 + \aheap_2'} \models \bigwedge_{\avariableter \in \asetter} n(\avariableter) = n(\overline{\avariableter})$. Indeed, $\asetter \subseteq \asetbis$, $\avariableter \in \asetter$,
and, $\astore_2(\avariableter)$ and $\astore_2(\overline{\avariableter})$ point to the same location. 
 %% \SDnote{There is something here in my notes, that I cannot decipher but I should do it when I am back.}
  Furthermore, $\pair{\astore_2}{\aheap_2 + \aheap_2'}$ also satisfies $\Safe(\aset)$ and therefore this entails that
  \[
  \pair{\astore_2}{\aheap_2 + \aheap_2'} \models (\bigwedge_{\avariableter \in \asetter}
   \alloc{\overline{\avariableter}} \wedge \size = \card{\asetter}) \separate
  \atranslation(\aformula_2, \aset).
  \]
  We have just seen that $\aheap_2 + \aheap_2'$ can be written as
  \[
    \aheap_1 + \aheap_1' + \{ \astore_2(\avariablebis) \pto \astore_1(\avariablebis) \mid \avariablebis \in \asetbis\} +
    \{\astore_2(\overline{\avariableter}) \pto \astore_1(\avariableter) \mid \avariableter \in \asetter\}.
  \]
  The formula $\bigwedge_{\avariableter \in \asetter} \alloc{\overline{\avariableter}} \wedge \size = \card{\asetter}$ can  be only  satisfied
  by  the memory state with the heap $\{\astore_2(\overline{\avariableter}) \pto \astore_1(\avariableter) \mid \avariableter \in
  \asetter\}$. Consequently, $\aheap_2 + \aheap_1'$ is equal to
  \[
    \aheap_1 + \aheap_1' + \{ \astore_2(\avariablebis) \pto \astore_1(\avariablebis) \mid \avariablebis \in \asetbis\},
  \]
  which entails that $\pair{\astore_2}{\aheap_2 + \aheap_1'} \models \atranslation(\aformula_2, \aset)$.
  Lastly, since $\triple{\LOC_1}{\astore_1}{\aheap_1 + \aheap_1'} \rhd^{\asetbis}_q \triple{\LOC_2}{\astore_2}{\aheap_2 + \aheap_1'}$,
  we can use the induction hypothesis to conclude that $\pair{\astore}{\aheap_1 + \aheap_1'} \models \aformula_2$.
  \qedhere
%% \qed
  \end{enumerate}
\end{proof}


==> proof-lemma-inverse-plus-alloc.tex <==
\begin{proof}
First, suppose that $\astore(\avariable) \in \range{\aheap}$. If $\aheap(\astore(\avariable)) = \astore(\avariable)$, then $\pair{\astore}{\aheap} \models
\avariable \hpto \avariable$ and obviously $\pair{\astore}{\aheap} \models \allocback{\avariable}$. Otherwise, let $\alocation \neq \astore(\avariable)$
be such that $\aheap(\alocation) = \astore(\avariable)$. The heap $\aheap' = \set{\alocation \mapsto \astore(\avariable)}$ satisfies
$\pair{\astore}{\aheap'} \models \new(\avariable) \septraction \reachplus(\avariable,\avariable) \wedge \size = 2 \wedge \neg ( \avariable \hpto \avariable)$
since $\pair{\astore}{\set{\astore(\avariable) \mapsto \alocation}} \models \new(\avariable)$
and $\pair{\astore}{\aheap' + \set{\astore(\avariable) \mapsto \alocation}}
\models (\reachplus(\avariable,\avariable) \wedge \size = 2 \wedge \neg ( \avariable \hpto \avariable)$.
Moreover, since $\card{\domain{\aheap'}} = 1$, we conclude that
 $\pair{\astore}{\aheap} \models [\new(\avariable) \septraction (\reachplus(\avariable,\avariable) \wedge \size = 2 \wedge \neg ( \avariable \hpto \avariable))]_1$.

Conversely, suppose that $\pair{\astore}{\aheap} \models \allocback{\avariable}$. If $\pair{\astore}{\aheap} \models
\avariable \hpto \avariable$, then obviously,  $\astore(\avariable) \in \range{\aheap}$. Otherwise, suppose that
$\pair{\astore}{\aheap} \models \neg (\avariable \hpto \avariable) \wedge
[\new(\avariable) \septraction (\reachplus(\avariable,\avariable) \wedge \size = 2 \wedge \neg ( \avariable \hpto \avariable))]_1$.
Therefore it must exist a one-memory-cell heap $\aheap' \sqsubseteq \aheap$ satisfying $\new(\avariable) \septraction (\reachplus(\avariable,\avariable) \wedge \size = 2 \wedge \neg ( \avariable \hpto \avariable))$.
Notice that this formula implies that $\astore(\avariable) \not\in \domain{\aheap'}$, since it should be possible to add a heap $\aheap''$ 
to $\aheap'$
such that $\pair{\astore}{\aheap''} \models \new(\avariable)$.
We distinguish three cases (picture below) of one-memory-cell heaps satisfying this property.
\begin{center}
  \begin{tikzpicture}[baseline]
    \node[dot,label=above:${\avariable}$] (l1) at (0,0) {};
    \node[dot] (l2) [right=0.5cm of l1] {};
    \node[dot] (l3) [below of=l2] {};

    \draw[pto] (l2) -- (l3);
  \end{tikzpicture}
  \qquad\qquad
    \begin{tikzpicture}[baseline]
      \node[dot,label=above:${\avariable}$] (l1) at (0,0) {};
      \node[dot] (l2) [right=0.5cm of l1] {};

      \draw[pto] (l2) edge [loop below, in=-30, out=-150,looseness=20] node {} (l2);
    \end{tikzpicture}
  \qquad
    \begin{tikzpicture}[baseline]
      \node[dot,label=above:${\avariable}$] (l1) at (0,0) {};
      \node[dot] (l2) [right=0.5cm of l1] {};

      \draw[pto] (l2) -- (l1);
    \end{tikzpicture}
\end{center}
The last memory state in the picture is the only that satisfies $\new(\avariable) \septraction (\reachplus(\avariable,\avariable) \wedge \size = 2 \wedge \neg ( \avariable \hpto \avariable))$. Indeed, by composing the other two heaps with a one-memory-cell heap satisfying $\new(\avariable)$ we cannot satisfy the formula $\reachplus(\avariable,\avariable)$. So, $\astore(\avariable) \in \range{\aheap}$.
%% \qed
\end{proof}


==> proof-lemma-next-pointstobis.tex <==
\begin{proof} 
%The only problem in the definition of $\aformula_{\hpto}^{+}(\avariable,\avariablebis)$ is the presence of $\reachplus$
%in the subformula $(\true \sepimp \lnot \reachplus(\avariable,\avariable))$. The formula
%$\aformula_{\hpto}(\avariable,\avariablebis, \avariableter)$ is obtained from
%$\aformula_{\hpto}^{+}(\avariable,\avariablebis)$  by replacing $(\true \sepimp \lnot \reachplus(\avariable,\avariable))$
%by $(\true \sepimp \lnot \reach(\avariable,\avariableter))$.
%
%The proof that for all the memory states $\pair{\astore}{\aheap}$ such that $\astore(\avariable) \neq \astore(\avariableter)$ and
%$\astore(\avariablebis) \neq \astore(\avariableter)$, we have
%$\pair{\astore}{\aheap} \models n(\avariable) \hpto  n(\avariablebis)$ iff
%$\pair{\astore}{\aheap} \models  \aformula_{\hpto}(\avariable,\avariablebis,\avariableter)$ is then very similar to the proof
%of Lemma~\ref{lemma-three-in-one}(I).
For (II), it is easy to show that $n(\avariable) \hpto n(\overline{\avariable})$ will never occur in the translation. Indeed, by always translating formulae with variables in $\{\avariable_1,\dots,\avariable_q\}$ we can only have $n(\avariable_i) \hpto n(\avariable_j)$ or $n(\overline{\avariable_i}) \hpto n(\overline{\avariable_j})$ (the latter case due to the renaming in the translation of the left side of the magic wand).
As such, $\aformula_{\hpto}(\avariable,\avariablebis, \overline{\avariable})$ can be used to check whenever $n(\avariable) \hpto n(\avariablebis)$.
\qed
\end{proof}


==> proof-lemma-sees.tex <==
\begin{proof}
 Suppose there exists a labelled location $\sem{v^{\star}}_{\astore,\aheap}$
that reaches a location $\alocation_i$ without reaching $\sem{v}_{\astore,\aheap}$, as shown in Figure~\ref{fig:sees}.
\begin{figure}
  \centering

  \begin{tikzpicture}
    \node[dot,label=below:$\sem{v}_{\astore,\aheap}$] (v1) at (0,0) {};
    \node[dot,label=below:$\ell_1$] (l1) [right of=v1] {};
    \node[dot,label=below:$\ell_i$,fill=red,red] (li) [right of=l1] {};
    \node[dot,label=below:$\ell_k$] (lk) [right of=li] {};
    \node[dot,label=below:$\sem{v'}_{\astore,\aheap}$] (v2) [right of=lk] {};
    \node[dot,label=right:$\sem{v^{\star}}_{\astore,\aheap}$] (v3) [above left of=li] {};

    \draw[pto] (v1) -- (l1);
    \draw[pto] (lk) -- (v2);

    \draw[reach] (l1) -- (li);
    \draw[reach] (li) -- (lk);
    \draw[reach] (v3) -- (li);
  \end{tikzpicture}
  \caption{If $\alocation_i \in \Reach^+(\sem{v^{\star}}_{\astore,\aheap})$  and $\sem{v^{\star}}_{\astore,\aheap}$
is not an  ancestor of
$\sem{v}_{\astore,\aheap}$, then $\alocation_i \in \Labels{q}{\astore,\aheap}$.}\label{fig:sees}
\end{figure}
 Then,  there exist two program variables $\avariable_i$ and $\avariable_j$, $i,j \in \interval{1}{q}$,
such that $\astore(\avariable_i)$ reaches $\sem{v}_{\astore,\aheap}$
(either $v = \avariable_i$, or $\sem{v}_{\astore,\aheap}$ is a meet-point and therefore reached by at least two other variables) and
$\astore(\avariable_j)$ reaches $\sem{v^{\star}}_{\astore,\aheap}$.
Moreover, there exists $\astore(\avariable_k)$ that is reached by $\sem{v'}_{\astore,\aheap}$
(either $v' = \avariable_k$ or $\sem{v'}_{\astore,\aheap}$ is a meet-point and therefore must reach a program variable).
 From the definition of meet-point, it must therefore hold that $\sem{m_q(\avariable_i,\avariable_j)}_{\astore,\aheap}= \alocation_i$
or $\sem{m_q(\avariable_j,\avariable_i)}_{\astore,\aheap} =\alocation_i$ and therefore $\alocation_i$ belongs to
$\Labels{q}{\astore,\aheap}$.
This is in contradiction with the hypotheses.
  \qed
\end{proof}


==> proof-theorem-last-decidability.tex <==
\begin{proof}
Let $\aformula$ be a formula in $\seplogic{\separate, \magicwand, \reachplus}$ in which $\reachplus$ is not
in the scope of $\magicwand$ 
and the program variables are among $\avariable_1$, \ldots, $\avariable_q$. The algorithm works as follows.
\begin{enumerate}
\itemsep 0 cm
\item For each maximal subformula $\aformulabis$ of $\aformula$ whose main connective is $\magicwand$ (and therefore
$\aformulabis$ is in $\seplogic{\separate, \magicwand}$), we compute a Boolean combination of test formulae
from those mentioned in Proposition~\ref{proposition-prop-sl}.  Actually Proposition~\ref{proposition-prop-sl} states
its existence but we can restrict ourselves to test formulae among 
$\size \geq \beta$ with $\beta \leq 2 \length{\aformula}$, $\alloc{\avariable_i}$,
$\avariable_i \pointsl{} \avariable_j$ and $\avariable_i = \avariable_j$ ($i,j \in \set{1,\ldots,q}$). 
One can enumerate the non-equivalent Boolean combinations $\aformulater$ built on those test formulae
and check in polynomial space in $\length{\aformulater} + \length{\aformulabis}$ whether
$\aformulater \Leftrightarrow \aformulabis$ is valid. Indeed, the validity problem for
$\seplogic{\separate, \magicwand}$ is in \pspace~\cite{Calcagno&Yang&OHearn01}. The enumeration
can be done in exponential space as well as the validity checking. 
\item  Let $\aformula'$ be the formula in  $\seplogic{\separate, \reachplus, \bigcup_{q,\alpha} \Test(q,\alpha)}$ obtained
       from $\aformula$ by replacing every maximal subformula $\aformulabis$  whose main connective is $\magicwand$
       by its equivalent Boolean combination with test formulae from $\Test(q,  2 \length{\aformula})$ by using  
       also Lemma~\ref{lemma-atomic-formulae-test} to eliminate the atomic formula of the form $\size \geq \beta$. The size of $\aformula'$ is exponential in $\length{\aformula}$
       and $\aformula'$ can be computed in exponential space in $\length{\aformula}$.
\item  Since the satisfiability problem for $\seplogic{\separate, \reachplus, \bigcup_{q,\alpha} \Test(q,\alpha)}$
       is in \pspace when the constants are encoded in unary and the maximal constant in  $\aformula'$ is $2 \length{\aformula}$,
       the satisfiability status of $\aformula'$ can be checked in polynomial space in $\aformula'$ and therefore
       in exponential space in $\length{\aformula}$. 
\end{enumerate}
Hence, the satisfiability problem is decidable and in \expspace according to the analysis above. \qed 
\end{proof}


==> section-other-fragments.tex <==
\section{Pushing the decidability border}

The content of this section is not yet determined. One option is to study
decidable fragments between $\seplogic{\separate\ls}$ and 
$\seplogic{\separate, \magicwand, \ls}$, for instance by restricting the polarity of the
$\magicwand$ or by having restrictions on the arguments of $\magicwand$. The other option,
which is probably the best, consists in providing the decidability status of 
$\seplogic{\magicwand, \ls}$.




==> section-undecidability.tex <==
\section{Undecidability of $\seplogic{\separate, \magicwand, \ls}$}%%
\label{section-undecidability}
In this section, we show that $\seplogic{\separate, \magicwand,\ls}$
has an undecidable satisfiability problem
even though it does not admit first-order quantification.%%
%%
\subsection{Principle of the reduction}%%
%%
Let  $\foseplogic{\magicwand}$ be the first-order extension of
$\seplogic{\magicwand}$ obtained by adding the universal quantifier $\forall$.
In the versions of $\foseplogic{\magicwand}$  defined in~\cite{Brochenin&Demri&Lozes12,DemriDeters16},
one distinguishes program variables from quantified variables (used with the quantifier $\forall$).
This distinction made by the two sets of variables is not necessary herein and for the sake of simplicity, we adopt
a version of   $\foseplogic{\magicwand}$ with a unique type of variables.
The formulae $\aformula$ of $\foseplogic{\magicwand}$ are built from from grammars below:
$$
\aatomicformula ::= \avariable = \avariablebis \ \mid \
                    \avariable \hpto \avariablebis$$
$$\aformula ::= \aatomicformula \ \mid \  \neg \aformula \ \mid \ \aformula \vee \aformula
               \ \mid \ \aformula \magicwand \aformula
               \ \mid \ \forall \avariable \ \aformula,$$
where $\avariable, \avariablebis \in \PVAR$.
Note that $\emptyconstant$ can be easily defined by $\forall \ \avariable, \avariable' \ \neg \avariable \hpto \avariable'$.
Models of the logic $\foseplogic{\magicwand}$ are
memory states and the satisfaction relation $\models$ is defined as for $\seplogic{\magicwand}$
with the clause:
$\pair{\astore}{\aheap} \models \forall \avariable \ \aformula$ $\iff$
  for all $\alocation \in \LOC$, we have $\pair{\astore[\avariable \leftarrow \alocation]}{\aheap} \models \aformula$.
Without any loss of generality, we can assume that the satisfiability (resp. valid) problem for
$\foseplogic{\magicwand}$ is defined by taking as inputs closed formulae (i.e. without free occurrences of the variables).

\begin{proposition}~\cite{Brochenin&Demri&Lozes12,DemriDeters16}
The satisfiability problem for $\foseplogic{\magicwand}$ is undecidable
and the set of valid formulae for $\foseplogic{\magicwand}$ is not recursively enumerable.
\end{proposition}%%
%%
\OnlyForVL{
The undecidability of $\foseplogic{\magicwand}$  with heaps having  at least two record fields
(i.e. $\aheap$ is of the form $\LOC \to_{\fin} \LOC^k$ with $k \geq 2$)
is established in~\cite{Calcagno&Yang&OHearn01}. Actually, $\magicwand$ is even not used in that
undecidability proof.}%% end of OnlyForVL
%%
In a nutshell, the undecidability of $\seplogic{\separate, \magicwand, \ls}$ is shown by reduction from
the satisfiability problem for  $\foseplogic{\magicwand}$. By definition, the satisfaction of the quantified formula $\forall \ \avariable \ \aformulabis$
from $\foseplogic{\magicwand}$ requires the satisfaction of the formula $\aformulabis$ for all the values in $\LOC$
assigned to $\avariable$.
This can be simulated in $\seplogic{\separate, \magicwand, \ls}$ by a formula of the form $(\alloc{\avariable} \wedge \size = 1) \magicwand
\atranslation(\aformulabis)$ where the right argument recursively calls the translation function and values for the universal quantification
are encoded in $\aheap(\astore(\avariable))$. In order to take adequately advantage of the universal quantification in the interpretation
of the separating implication $\magicwand$, we present below our approach and the obstacles we have to avoid.
\begin{enumerate}
\itemsep 0 cm
\item A memory state satisfies the formula $(\alloc{\avariable} \wedge \size = 1) \magicwand \atranslation(\aformulabis)$ in a non-trivial
way only if it does not satisfy $\alloc{\avariable}$. Consequently, in the translation process, if a closed formula $\aformula$ in $\foseplogic{\magicwand}$
contains quantifications over variables in $\aset = \set{\avariable_1, \ldots, \avariable_q}$, its translation in $\seplogic{\separate, \magicwand, \ls}$ should be roughly
of the form
$
(\bigwedge_{i} \neg \alloc{\avariable_i}) \wedge
(\bigwedge_{i \neq j} \avariable_i \neq \avariable_j) \wedge
(\bigwedge_{i,j} \neg \avariable_i \hpto \avariable_j) \wedge \atranslation(\aformula)
$.
This assumes also that two distinct quantifications in $\aformula$ are performed on distinct variables (easy to guarantee
with adequate renaming).
\item The third generalised conjunction $(\bigwedge_{i,j} \neg \avariable_i \hpto \avariable_j)$ may come as a surprise but
the values for the variables $\avariable_1$, \ldots, $\avariable_q$, should not interfere with the other part of the heap
and more generally, at any stage of the translation one should guarantee that each variable $\avariable_i$ is also not interpreted
by a location in the heap range. That is why, we require that the atomic formula $\allocback{\avariable}$ can be expressed
in some way, where $\pair{\astore}{\aheap} \models \allocback{\avariable}$ $\iff$ $\astore(\avariable)  \in \range{\aheap}$.
So, we write ${\rm OK}(\aset)$ to denote
$
(\bigwedge_{i \neq j} \avariable_i \neq \avariable_j) \wedge
(\bigwedge_{i,j} \neg \avariable_i \hpto \avariable_j) \wedge
(\bigwedge_{i} \neg \allocback{\avariable_i})
$
and the translation of the formula $\aformula$ would simply become
$(\bigwedge_{i} \neg \alloc{\avariable_i}) \wedge {\rm OK}(\aset) \Rightarrow \atranslation(\aformula)$
(beware that some further refinements are needed actually).
It remains to prove that $\allocback{\avariable_i}$ can be expressed in this context, see Lemma~\ref{lemma-allocback}.
\item More generally, whenever a subheap is added thanks to  $\magicwand$, one needs to check that ${\rm OK}(\aset)$ holds true afterwards.
      For instance, the translation of $\forall \ \avariable \ \aformulabis$ will be of the form $(\alloc{\avariable} \wedge \size = 1) \magicwand
({\rm OK}(\aset) \implies \atranslation(\aformulabis))$.
\item The encoding of the value $\astore(\avariable)$ in  $\foseplogic{\magicwand}$ by the value $\aheap(\astore(\avariable))$ in
$\seplogic{\separate, \magicwand, \ls}$ requires that we can express in the target logic the atomic formula $n(\avariable) = n(\avariablebis)$ defined
by $\pair{\astore}{\aheap} \models n(\avariable) = n(\avariablebis)$ $\iff$ $\astore(\avariable),\astore(\avariablebis) \in \domain{\aheap}$
and $\aheap(\astore(\avariable)) = \aheap(\astore(\avariablebis))$. Indeed, the translation of $\avariable = \avariablebis$ should be precisely
$n(\avariable) = n(\avariablebis)$.
This atomic formula cannot be expressed in $\seplogic{\separate, \magicwand}$
(see Proposition~\ref{proposition-prop-sl})
but fortunately,
it can be done in $\seplogic{\separate, \magicwand, \ls}$ (see Lemma~\ref{lemma-three-in-one}(I)).
\item In the same vein,  the translation of $\avariable \hpto \avariablebis$ could be the new atomic formula
$n(\avariable) \hpto n(\avariablebis)$ (or  a formula equivalent to it) where
$\pair{\astore}{\aheap} \models n(\avariable) \hpto n(\avariablebis)$ $\iff$ $\astore(\avariable),\astore(\avariablebis) \in \domain{\aheap}$
and $\aheap(\aheap(\astore(\avariable))) = \aheap(\astore(\avariablebis))$. Fortunately, it can be expressed in $\seplogic{\separate, \magicwand, \reachplus}$
(see Lemma~\ref{lemma-three-in-one}(II)). As far as  $\seplogic{\separate, \magicwand, \ls}$ is concerned, this new atomic formula can be also expressed
in it but we need
an auxiliary variable (see Lemma~\ref{lemma-three-in-one}(III)). Using an additional variable is not too bad as demonstrated in the
sequel.
\item Last but not least, the translation of a formula $\aformulabis_1 \magicwand \aformulabis_2$ cannot simply be of the form
$\atranslation(\aformulabis_1) \magicwand ({\rm OK}(\aset) \Rightarrow \atranslation(\aformulabis_2))$ because the evaluation of $\atranslation(\aformulabis_1)$
in a disjoint heap may need the values of free variables occurring in $\aformulabis_1$ but our encoding  of the variable valuations via the heap
does not allow to preserve these values through disjoint heaps. In order to solve this problem, we introduce an auxiliary set of
variables  $\bar{\aset} = \set{\bar{\avariable}_1, \ldots, \bar{\avariable}_q}$ made of copies of variables from $\aset$ that are allocated
on the left side of the magic wand, and checked to be equal to their non-bar versions on the right side of the magic wand.
The translation of $\aformulabis_1 \magicwand \aformulabis_2$ is then of the form
$$
((\bigwedge_{\avariablebis \in \asetter} \alloc{\bar{\avariablebis}}) \wedge (\bigwedge_{\avariableter \in (\aset \cup \bar{\aset}) \setminus \asetter} \neg \alloc{\avariableter})
\wedge {\rm OK}(\asetter) \wedge \atranslation(\aformulabis_1)[\avariable \leftarrow \bar{\avariable}])
\magicwand
$$
$$ (((\bigwedge_{\avariablebis \in \asetter} n(\avariablebis) = n(\bar{\avariablebis})) \wedge {\rm OK}(\aset \cup \bar{\aset}))
   \Rightarrow
((\bigwedge_{\avariablebis \in \asetter} \alloc{\bar{\avariablebis}} \wedge \size = \card{\asetter}) \separate \atranslation(\aformulabis_2)))
$$
where $\asetter \subseteq \aset$ is the set of free variables in $\aformulabis_1$.
The formula $\atranslation(\aformulabis_1)[\avariable \leftarrow \bar{\avariable}]$
is defined from $\atranslation(\aformulabis_1)$ by replacing every variable $\avariable_i$ by $\bar{\avariable}_i$.
The first conjuncts of the left argument guarantee that
auxiliary variables are assigned values to evaluate $\atranslation(\aformulabis_1)[\avariable \leftarrow \bar{\avariable}]$.
In the right argument $\magicwand$,
the antecedent of the (material) implication insures that
a variable and its copy point to the same value (necessary for a proper evaluation of the formula $ \atranslation(\aformulabis_1)[\avariable \leftarrow \bar{\avariable}]$)
whereas the conclusion of the implication ensures that $\atranslation(\aformulabis_2)$ is evaluated
on a heap in which the copy variables are unallocated, providing an economical variable recycling.
In order to fully take into account the auxiliary variables, the top translation becomes
$
(\bigwedge_{i} \neg \alloc{\avariable_i} \wedge  \neg \alloc{\bar{\avariable}_i}) \wedge {\rm OK}(\aset \cup \bar{\aset}) \wedge \atranslation(\aformula)
$.
\end{enumerate}%%
%%
Below, we provide  the technical developments to validate this proof strategy.%%
%%
\subsection{The translation}%%
First, we briefly explain how to express the formulae $\allocback{\avariable}$,
$n(\avariable) =  n(\avariablebis)$ and $n(\avariable) \rightarrow  n(\avariablebis)$ within
$\seplogic{\separate, \magicwand, \ls}$ or $\seplogic{\separate, \magicwand, \reachplus}$
(see also the proofs in the technical appendix).
%%
Let us introduce a few macros that shall be helpful.%%
\begin{itemize}
\itemsep 0 cm
\item Given $\aformula$ in $\seplogic{\separate, \magicwand, \reachplus}$ and $n \geq 0$, we write
$[\aformula]_n$ to denote  $(\size = n \land \aformula) \separate \true$. It is easy to show that
for all memory states $\pair{\astore}{\aheap}$, we have $\pair{\astore}{\aheap} \models [\aformula]_n$
iff there is  $\aheap' \sqsubseteq \aheap$ such that $\card{\domain{\aheap'}} = n$ and
$\pair{\astore}{\aheap'} \models \aformula$.
\OnlyForVL{
Such formulae $[\aformula]_n$ can be used to ensure that the minimum path between two locations interpreted by
program variables is of length $n$.
}%% End OnlyForVL
We write $\reach(\avariable,\avariablebis) = n$ to denote the formula $[\ls(\avariable,\avariablebis)]_n$.%%
%%
\item Given variables $\avariable_1$, \ldots, $\avariable_{\gamma}$, below we introduce the formula $\new(\avariable_1,\dots,\avariable_{\gamma})$
$$
\size = \gamma \land \bigwedge_{i \in \interval{1}{\gamma}} (\alloc{\avariable_i} \land (\bigwedge_{j \in \interval{1}{\gamma}}
\neg \avariable_i \hpto \avariable_j) \land (\bigwedge_{j \neq i \in \interval{1}{\gamma}}
\avariable_i \neq \avariable_j)).
$$
\end{itemize}%%
%%
Let us define $\allocback{\avariable}$ as
$
\avariable \hpto \avariable \vee [\new(\avariable) \septraction (\reachplus(\avariable,\avariable) \wedge \size = 2 \wedge \neg ( \avariable \hpto \avariable))]_1$, and
the lemma below states that the formula $\allocback{\avariable}$ does the job.%%
%%
\begin{lemma}
\label{lemma-allocback}
For all
%% memory states
$\pair{\astore}{\aheap}$, we have $\pair{\astore}{\aheap} \models \allocback{\avariable}$ iff $\astore(\avariable) \in \range{\aheap}$.
\end{lemma}%%
%%
\OnlyForVL{\input{proof-lemma-inverse-plus-alloc}}%%
%%
In order to define the existence of a predecessor in  $\seplogic{\separate, \magicwand, \reach}$ (this time we cannot use
$\reachplus$ anymore), we need to take advantage of
an auxiliary variable $\avariablebis$ whose value is different from the one for $\avariable$. Let $\mathtt{alloc}_{\avariablebis}^{-1}(\avariable)$ be the formula
$
\avariable \hpto \avariable \vee \avariablebis \hpto \avariable \vee
[\neg \alloc{\avariablebis} \wedge (\alloc{\avariablebis} \land \lnot \avariablebis \hpto \avariable \land \size = 1 ) \lollipop \reach(\avariablebis,\avariable)]_1$.

\begin{lemma}
\label{lemma-inverse-alloc}
For all memory states $\pair{\astore}{\aheap}$ such that $\astore(\avariable) \neq \astore(\avariablebis)$,
we have $\pair{\astore}{\aheap} \models \mathtt{alloc}_{\avariablebis}^{-1}(\avariable)$ iff $\astore(\avariable) \in \range{\aheap}$.
\end{lemma}%%
%%
\OnlyForVL{\input{proof-lemma-inverse-alloc}}%%
%%
%%
Other essential properties are stated below.%%
%%
\begin{lemma}
\label{lemma-three-in-one}
Let $\avariable, \avariablebis, \avariableter \in \PVAR$.
(I) There is $\aformula_{=}(\avariable,\avariablebis)$
in $\seplogic{\separate, \magicwand, \ls}$
such that $n(\avariable) =  n(\avariablebis) \equiv \aformula_{=}(\avariable,\avariablebis)$.
(II) There is $\aformula_{\hpto}^{+}(\avariable,\avariablebis)$
in $\seplogic{\separate, \magicwand, \reachplus}$
such that
$n(\avariable) \hpto  n(\avariablebis) \equiv
\aformula_{\hpto}^{+}(\avariable,\avariablebis)$.
(III) There is  $\aformula_{\hpto}(\avariable,\avariablebis, \avariableter)$
in $\seplogic{\separate, \magicwand, \ls}$
such that
$
\avariable \neq \avariableter \wedge \avariablebis \neq \avariableter \wedge n(\avariable) \hpto  n(\avariablebis) \equiv
\avariable \neq \avariableter \wedge \avariablebis \neq \avariableter  \wedge \aformula_{\hpto}(\avariable,\avariablebis,\avariableter)
$.
\end{lemma}
%%
%% SD 15/10/2017
%%
%% One lemma for three.
%%
\OnlyForVL{
\begin{lemma}
\label{lemma-next-equality}
Let $\avariable, \avariablebis \in \PVAR$. There is a formula $\aformula_{=}(\avariable,\avariablebis)$
in $\seplogic{\separate, \magicwand, \ls}$ (or equivalently in  $\seplogic{\separate, \magicwand, \reach}$)
such that $n(\avariable) =  n(\avariablebis) \equiv \aformula_{=}(\avariable,\avariablebis)$.
\end{lemma}%%
%%
\OnlyForVL{\input{proof-lemma-next-equality}}%%
%%
\begin{lemma}
\label{lemma-next-pointsto}
Let $\avariable, \avariablebis \in \PVAR$. There is a formula $\aformula_{\hpto}^{+}(\avariable,\avariablebis)$
in $\seplogic{\separate, \magicwand, \reachplus}$
such that
$n(\avariable) \hpto  n(\avariablebis) \equiv
\aformula_{\hpto}^{+}(\avariable,\avariablebis)$.
\end{lemma}
%%
\OnlyForVL{\input{proof-lemma-next-pointsto}}%%
%%
\begin{lemma}
\label{lemma-next-pointstobis}
Let $\avariable, \avariablebis, \avariableter \in \PVAR$. There is a formula $\aformula_{\hpto}(\avariable,\avariablebis, \avariableter)$
in $\seplogic{\separate, \magicwand, \ls}$
such that
$
\avariable \neq \avariableter \wedge \avariablebis \neq \avariableter \wedge n(\avariable) \hpto  n(\avariablebis) \equiv
\avariable \neq \avariableter \wedge \avariablebis \neq \avariableter  \wedge \aformula_{\hpto}(\avariable,\avariablebis,\avariableter)
$.
\end{lemma}
}%% End of OnlyForVL
Lemma~\ref{lemma-three-in-one}(III) is equivalent to:
for all the memory states $\pair{\astore}{\aheap}$ such that $\astore(\avariable) \neq \astore(\avariableter)$ and
$\astore(\avariablebis) \neq \astore(\avariableter)$, we have
$\pair{\astore}{\aheap} \models n(\avariable) \hpto  n(\avariablebis)$ iff
$\pair{\astore}{\aheap} \models  \aformula_{\hpto}(\avariable,\avariablebis,\avariableter)$.%%
%%
\OnlyForVL{\input{proof-lemma-next-pointstobis}}%%
%%

The importance of the Lemmas~\ref{lemma-allocback}--\ref{lemma-three-in-one} should not be neglected.
Indeed, these results state that relatively simple properties can be expressed in the logic
$\seplogic{\separate, \magicwand, \ls}$ and the like but this is essential to perform
the translation.\\
%%
%%
Let $\aset = \set{\avariable_1, \ldots, \avariable_{2q}}$ be a  set of program variables with $q \geq 2$.
We define the map $\bar{\ \cdot \ }: \aset \rightarrow \aset$ so that
for all $i \in \interval{1}{q}$, we have $\bar{\avariable}_i \egdef \avariable_{i+q}$ and
$\bar{\avariable}_{i+q} \egdef \avariable_{i}$.
We write ${\rm OK}(\aset)$ to denote the formula
$
(\bigwedge_{i \neq j} \avariable_i \neq \avariable_j) \wedge
(\bigwedge_{i,j} \neg \avariable_i \hpto \avariable_j) \wedge
(\bigwedge_{i}  \neg \mathtt{alloc}_{\bar{\avariable}_{i}}^{-1}(\avariable_i))
$.
%%
Let $\aformula$ be a closed formula in $\foseplogic{\magicwand}$ with quantified variables in
$\set{\avariable_1, \ldots, \avariable_q}$.
W.l.o.g., we can assume that $q \geq 2$ and two distinct quantifications involve distinct variables.
We define below the translation $\mathcal{T}_{\rm SAT}(\aformula)$ in $\seplogic{\separate, \magicwand, \ls}$ where
$\atranslation(\aformula, \aset)$ is defined recursively.
$$
\mathcal{T}_{\rm SAT}(\aformula) \egdef
(\bigwedge_{i \in \interval{1}{2q}} \neg \alloc{\avariable_i}) \wedge {\rm OK}(\aset) \wedge \atranslation(\aformula, \aset).
$$%%
The first two conjuncts specify initial conditions, namely each variable $\avariablebis$ in $\aset$
is interpreted by a location that is unallocated, it is not in the  heap range and it is distinct from the interpretation of
all other variables; otherwise said, the value for $\avariablebis$ is isolated.
The translation function $\atranslation$ has two arguments: the formula in $\foseplogic{\magicwand}$ to be recursively translated
and the total set of variables potentially appearing in the target formula (useful to check that ${\rm OK}(\aset)$
holds on every heap involved in the satisfaction of the translated formula).
Note also that the translation shall be performed into the target logic $\seplogic{\separate, \magicwand, \ls}$,
which can be viewed as a
fragment of
$\seplogic{\separate, \magicwand, \reachplus}$.
The introduction of the formulae in $\seplogic{\separate, \magicwand, \reachplus}$ has been instrumental
to introduce those for  $\seplogic{\separate, \magicwand, \ls}$, sometimes at the cost of requiring additional variables.
Here, these additional variables are directly picked from $\aset$
and therefore there is no need to introduce new extra variables as soon as $q \geq 2$.

Let us come back to the  definition of $\atranslation(\aformulabis, \aset)$ (homomorphic for Boolean connectives) with the assumption
that the variables  in $\aformulabis$ are among $\avariable_1$, \ldots, $\avariable_q$.
\vspace*{-0.12in}
\begin{align*}
\atranslation(\avariable_i = \avariable_j, \aset) & \egdef \aformula_{=}(\avariable_i, \avariable_j)  \\
\atranslation(\avariable_i \hpto \avariable_j, \aset) & \egdef \aformula_{\hpto}(\avariable_i, \avariable_j, \bar{\avariable}_i)  \\
\atranslation(\forall \avariable_i \ \aformulabis, \aset) & \egdef (\alloc{\avariable_i} \wedge \size = 1) \magicwand
({\rm OK}(\aset) \Rightarrow
\atranslation(\aformulabis, \aset))
%%
%% \atranslation(\aformulabis_1 \wedge \aformulabis_2, \aset) & \egdef   \atranslation(\aformulabis_1,\aset) \wedge
%% \atranslation(\aformulabis_2,\aset) \\
%% \atranslation(\neg \aformulabis, \aset) & \egdef   \neg \atranslation(\aformulabis,\aset) \\
%%
\end{align*}%%
%%
Lastly, the translation $\atranslation(\aformulabis_1 \magicwand \aformulabis_2, \aset)$  is defined as
$$
((\bigwedge_{\avariablebis \in \asetter} \alloc{\bar{\avariablebis}}) \wedge
(\bigwedge_{\avariableter \in \aset \setminus \asetter} \neg \alloc{\bar{\avariableter}})
\wedge {\rm OK}(\aset) \wedge \atranslation(\aformulabis_1,\aset)[\avariable \leftarrow \bar{\avariable}])
\magicwand
$$
$$ (((\bigwedge_{\avariablebis \in \asetter} n(\avariablebis) = n(\bar{\avariablebis})) \wedge {\rm OK}(\aset))
   \Rightarrow
((\bigwedge_{\avariablebis \in \asetter} \alloc{\bar{\avariablebis}} \wedge \size = \card{\asetter}) \separate
\atranslation(\aformulabis_2, \aset))),
$$
where $\asetter \subseteq \set{\avariable_1, \ldots, \avariable_q}$ is the set of free variables in $\aformulabis_1$.
Below, we shall establish that $\aformula$ and $\mathcal{T}_{\rm SAT}(\aformula)$ are equisatisfiable.
Similarly, let $\mathcal{T}_{\rm VAL}(\aformula)$ be the formula in $\seplogic{\separate, \magicwand, \ls}$
defined by
$((\bigwedge_{i \in \interval{1}{2q}} \neg \alloc{\avariable_i}) \wedge {\rm OK}(\aset)) \Rightarrow
\atranslation(\aformula, \aset)$. As a consequence, $\aformula$ and $\mathcal{T}_{\rm VAL}(\aformula)$ are shown equivalid.%%
%%
%%
\subsection{The correctness proof}%%
%%
Below, we consider a slight alternative
for the semantics of the logics $\foseplogic{\magicwand}$ and $\seplogic{\separate,\magicwand,\ls}$,
which does not modify the notion of satisfiability/validity and such that
the set of formulae and
the definition of the satisfaction relation
$\models$ remain unchanged.
So far, the memory states are pairs of the form $\pair{\astore}{\aheap}$ with
$\astore: \PVAR \rightarrow \LOC$  and $\aheap: \LOC \to_{\fin} \LOC$  for a {\em fixed} countably infinite set of locations $\LOC$, say $\LOC = \Nat$.
Alternatively, the models for  $\foseplogic{\magicwand}$ and $\seplogic{\separate,\magicwand,\ls}$ can be defined
as triples $\triple{\LOC_1}{\astore_1}{\aheap_1}$ such that $\LOC_1$ is a countable infinite set,
$\astore_1: \PVAR \rightarrow \LOC_1$  and $\aheap_1: \LOC_1 \to_{\fin} \LOC_1$. As shown below, this does not
change the notion of satisfiability and validity, but this generalisation will be handy in a few places.
Most of the time, a generalised memory state $\triple{\LOC_1}{\astore_1}{\aheap_1}$ shall be written
$\pair{\astore_1}{\aheap_1}$ when no confusion is possible.

Given a bijection $\amap: \LOC_1 \rightarrow \LOC_2$ and a heap $\aheap_1: \LOC_1 \to_{\fin} \LOC_1$ equal to
$\set{\alocation_1 \mapsto \aheap_1(\alocation_1), \ldots,\alocation_n \mapsto \aheap_1(\alocation_n)}$,
we write $\amap(\aheap_1)$ to denote the heap  $\aheap_2: \LOC_2 \to_{\fin} \LOC_2$ with
$\aheap_2 = \set{\amap(\alocation_1) \mapsto \amap(\aheap_1(\alocation_1)), \ldots, \amap(\alocation_n) \mapsto \amap(\aheap_1(\alocation_n))}$.


\begin{definition}\label{def:partial_memory_state_iso}
Let $\triple{\LOC_1}{\astore_1}{\aheap_1}$ and  $\triple{\LOC_2}{\astore_2}{\aheap_2}$ be generalised
memory sta\-tes and $\aset \subseteq \PVAR$. A \defstyle{partial isomorphism} with respect to $\aset$
from  $\triple{\LOC_1}{\astore_1}{\aheap_1}$ to  $\triple{\LOC_2}{\astore_2}{\aheap_2}$ is a bijection
$\amap: \LOC_1 \rightarrow \LOC_2$ such that
$\aheap_2 = \amap(\aheap_1)$ and for all $\avariable \in \aset$,  $\amap(\astore_1(\avariable)) = \astore_2(\avariable)$
(we write $\triple{\LOC_1}{\astore_1}{\aheap_1} \approx_{\aset}  \triple{\LOC_2}{\astore_2}{\aheap_2}$).
%%
%% SD 12/10/2017
%% the conditions below hold:
%% \begin{itemize}
%% \itemsep 0 cm
%% \item for all $\avariable \in \aset$,  $\amap(\astore_1(\avariable)) = \astore_2(\avariable)$,
%% \item $\aheap_2 = \amap(\aheap_1)$.
%% %% \item for all $\alocation \in \LOC_1$,  $\alocation \in \domain{\aheap_1}$ iff $\amap(\alocation) \in \domain{\aheap_2}$
%% %% and if $\alocation \in \domain{\aheap_1}$, then $\amap(\aheap_1(\alocation)) = \aheap_2(\amap(\alocation))$,
%% %% \item for all $\alocation \in \LOC_2$, $\alocation \in \domain{\aheap_2}$ iff $\amap^{-1}(\alocation) \in \domain{\aheap_1}$
%% %% and if $\alocation \in \domain{\aheap_2}$, then $\amap^{-1}(\aheap_2(\alocation)) = \aheap_1(\amap^{-1}(\alocation))$.
%% \end{itemize}
\end{definition}%%
\OnlyForVL{
Note that if $\amap$ is a partial isomorphism from $\triple{\LOC_1}{\astore_1}{\aheap_1}$ to  $\triple{\LOC_2}{\astore_2}{\aheap_2}$,
then $\amap^{-1}$ is also a partial isomorphism from  $\triple{\LOC_2}{\astore_2}{\aheap_2}$ to  $\triple{\LOC_1}{\astore_1}{\aheap_1}$.
}
\OnlyForVL{
Two generalised memory states $\triple{\LOC_1}{\astore_1}{\aheap_1}$ and  $\triple{\LOC_2}{\astore_2}{\aheap_2}$
are said to be \defstyle{isomorphic with respect to $\aset$}, written $\triple{\LOC_1}{\astore_1}{\aheap_1} \approx_{\aset}
\triple{\LOC_2}{\astore_2}{\aheap_2}$, if and only if there exists a partial isomorphism w.r.t. $\aset$ between them.
}%% end OnlyForVL
\OnlyForVL{It is easy to check that $\approx_{\aset}$ is an equivalence relation.}%%
%%
A folklore result states that isomorphic memory states satisfy the same formulae
since the logics $\foseplogic{\magicwand}$, $\seplogic{\separate,\magicwand,\ls}$  can only
perform equality tests.
\OnlyForVL{
 between program variables interpreted by locations. Below, we state the precise result
we need in the sequel, the proof being by a standard  induction on the formula structure.}%%
%%
\begin{lemma}
\label{lemma-equivalence-isomorphism}
Let $\triple{\LOC_1}{\astore_1}{\aheap_1}$ and  $\triple{\LOC_2}{\astore_2}{\aheap_2}$ be generalised memory states
such that  $\triple{\LOC_1}{\astore_1}{\aheap_1} \approx_{\aset}  \triple{\LOC_2}{\astore_2}{\aheap_2}$, for some $\aset
\subseteq \PVAR$. (I) For all formulae $\aformula$ in  $\seplogic{\separate,\magicwand,\ls}$ built on variables among
$\aset$, we have $\triple{\LOC_1}{\astore_1}{\aheap_1} \models \aformula$ iff $\triple{\LOC_2}{\astore_2}{\aheap_2} \models \aformula$.
(II) For all formulae $\aformula$ in  $\foseplogic{\magicwand}$ whose free variables are  among
$\aset$, we have $\triple{\LOC_1}{\astore_1}{\aheap_1} \models \aformula$ iff $\triple{\LOC_2}{\astore_2}{\aheap_2} \models \aformula$.
\end{lemma}%%
%%
\OnlyForVL{\input{proof-lemma-equivalence-isomorphism}}%%
%%
As a direct consequence, satisfiability in  $\seplogic{\separate,\magicwand,\ls}$  as defined in Section~\ref{section-preliminaries}
is equivalent to satisfiability with generalised memory states, the same holds for $\foseplogic{\magicwand}$. Next,
we design a binary relation $\rhd_n^{\asetbis}$ between generalised memory states for $\foseplogic{\magicwand}$
and generalised memory states for $\seplogic{\separate,\magicwand,\ls}$ that is the semantical counterpart of the
syntactical translation process. Such a relation is parameterised by
$\set{\avariable_1, \ldots, \avariable_{2q}}$ (simply materialised by  $q$ below) and by a subset $\asetbis$ of free variables.
Then, Lemma~\ref{lemma-correctness-translation} relates   $\rhd_q^{\asetbis}$ and the map
$\atranslation$.


Given $\aset = \set{\avariable_1, \ldots, \avariable_{2q}}$, $\asetbis \subseteq \set{\avariable_1, \ldots, \avariable_{q}}$,
$\triple{\LOC_1}{\astore_1}{\aheap_1}$ and  $\triple{\LOC_2}{\astore_2}{\aheap_2}$
with $q \geq 2$, we write  $\triple{\LOC_1}{\astore_1}{\aheap_1} \rhd_q^{\asetbis} \ \triple{\LOC_2}{\astore_2}{\aheap_2}$
when (1)--(5) hold:%%
\begin{enumerate}
\itemsep 0 cm
\item[(1)] $\pair{\astore_2}{\aheap_2} \models {\rm OK}(\aset)$;
     (2) $\LOC_1 = \LOC_2 \setminus \set{\astore_2(\avariable) \ \mid \ \avariable \in \aset}$,
\item[(3)] the heap $\aheap_1$ is equal to the restriction of $\aheap_2$ to locations in $\LOC_1$,
\item[(4)] for all $\avariablebis \in \aset \setminus \asetbis$, $\astore_2(\avariablebis) \not \in \domain{\aheap_2}$;
     (5) for all $\avariablebis \in \asetbis$, $\aheap_2(\astore_2(\avariablebis)) = \astore_1(\avariablebis)$.
\end{enumerate}%%
%%
So, $\aheap_2$ is equal $\aheap_1 + \aheap_2'$ with $\aheap_2' = \set{\astore_2(\avariablebis) \pto \astore_1(\avariablebis) \mid \avariablebis \in \asetbis}$ and as such, by the condition (5.), $\aheap_2'$ encodes the store $\astore_1$. Therefore, the following result holds.

\begin{lemma}\label{lemma-rhd}
  Let $\aset = \set{\avariable_1, \ldots, \avariable_{2q}}$, $\asetbis \subseteq \set{\avariable_1, \ldots, \avariable_{q}}$ and,
  $\triple{\LOC_1}{\astore_1}{\aheap_1}$ and $\triple{\LOC_1}{\astore_2}{\aheap_2}$
  be two generalised memory states such that
  $\LOC_1 = \LOC_2 \setminus \set{\astore_2(\avariable) \ \mid \ \avariable \in \aset}$ and
  for all $\avariable_i \neq\avariable_j \in \aset$, we have  $\astore_2(\avariable_i) \neq \astore_2(\avariable_j)$.
  Then, $\triple{\LOC_1}{\astore_1}{\aheap_1} \rhd_q^{\asetbis} \ \triple{\LOC_2}{\astore_2}{\aheap_2}$
  iff $\aheap_2 = \aheap_1 + \set{\astore_2(\avariablebis) \pto \astore_1(\avariablebis)  \ \mid \ \avariablebis \in \asetbis}$.
\end{lemma}

Here is  the main result of this section, which is essential for the correctness of $\mathcal{T}_{\rm SAT}(\aformula)$
(see Appendix~\ref{appendix-proof-lemma-correctness-translation} for the proof using all the introduced ingredients).

\begin{lemma}
\label{lemma-correctness-translation}
Let  $\aset = \set{\avariable_1, \ldots, \avariable_{2q}}$,
$\asetbis \subseteq \{\avariable_1, \ldots, \avariable_q\}$,
$\aformulabis$
be a formula in $\foseplogic{\magicwand}$ with free variables among $\asetbis$ that
does not contain any bound variable of $\aformulabis$
and
 $\triple{\LOC_1}{\astore_1}{\aheap_1} \rhd_q^{\asetbis} \ \triple{\LOC_2}{\astore_2}{\aheap_2}$. We have
$\pair{\astore_1}{\aheap_1}  \models \aformulabis$ iff $\pair{\astore_2}{\aheap_2} \models \atranslation(\aformulabis,\aset)$.
\end{lemma}%%
%%
\OnlyForVL{\input{proof-lemma-correctness-translation}}%%
%%
Here is the important corollary.%%
%%
\begin{corollary}
\label{corollary-satisfiability-validity}
Let $\aformula$ be a closed formula in $\foseplogic{\magicwand}$ using quantified variables
among $\set{\avariable_1, \ldots, \avariable_q}$ with $q \geq 2$. (I)
$\aformula$ and $\mathcal{T}_{\rm SAT}(\aformula)$ are equisatisfiable.
(II) $\aformula$ and $\mathcal{T}_{\rm VAL}(\aformula)$ are equivalid.\end{corollary}%%
%%
\OnlyForVL{\input{proof-corollary-satisfiability-validity}}%%
%%
\subsection{Undecidability results and non-finite axiomatization}%%
%%
It is time to collect the fruits of all our efforts and to conclude this part about undecidability.
As a direct consequence of Corollary~\ref{corollary-satisfiability-validity} and the undecidability of
$\foseplogic{\magicwand}$, here is one of the main results of the paper.%%
%%
\begin{theorem}
\label{theorem-main-undecidability}
The satisfiability problem for $\seplogic{\separate, \magicwand, \ls}$ is undecidable.
\end{theorem}%%
%%
As a by-product, the set of valid formulae for  $\seplogic{\separate, \magicwand, \ls}$ is not
recursively enumerable.
Indeed, suppose that the set of valid formulae for $\seplogic{\separate, \magicwand, \ls}$
were r.e., then one can enumerate the valid formulae of the form $\mathcal{T}_{\rm VAL}(\aformula)$
as it is decidable in \ptime whether $\aformulabis$ in $\seplogic{\separate, \magicwand, \ls}$
is syntactically equal to  $\mathcal{T}_{\rm VAL}(\aformula)$ for some $\foseplogic{\magicwand}$ formula $\aformula$ with at least two variables.
This leads to a contradiction since this would allow the enumeration of valid formulae in $\foseplogic{\magicwand}$ with at least two variables.


The essential ingredients to establish the undecidability of $\seplogic{\separate, \magicwand, \ls}$
are the fact that the following properties $n(\avariable) = n(\avariablebis)$, $n(\avariable) \hpto n(\avariablebis)$
and $\allocback{\avariable}$ are expressible in the logic.

\begin{corollary}
\label{corollary-two-in-one}
$\seplogic{\separate, \magicwand}$ augmented with
built-in  formulae
of the form $n(\avariable) = n(\avariablebis)$, $n(\avariable) \hpto n(\avariablebis)$ and
$\allocback{\avariable}$ (resp. of the form $\reach(\avariable,\avariablebis) = 2$ and $\reach(\avariable,\avariablebis) = 3$)
admits an undecidable satisfiability problem.
\end{corollary}%%
%%
%%
\OnlyForVL{
\begin{corollary}
\label{corollary-undecidability-next}
$\seplogic{\separate, \magicwand}$ augmented with
built-in  formulae
of the form $n(\avariable) = n(\avariablebis)$, $n(\avariable) \hpto n(\avariablebis)$ and
$\allocback{\avariable}$
admits an undecidable satisfiability problem.
\end{corollary}

Corollary~\ref{corollary-undecidability-next} can be refined a bit further by noting in which context
the reachability predicates
$\ls$ and $\reach$ are used in the formulae. This allows us to get the result below by massaging
a bit the formulae built so far.

\begin{corollary}
\label{corollary-undecidability-limited-reach}
$\seplogic{\separate, \magicwand}$ augmented with
built-in formulae
of the form $\reach(\avariable,\avariablebis) = 2$ and $\reach(\avariable,\avariablebis) = 3$
admits an undecidable satisfiability problem.
\end{corollary}
}%% OnlyForVL
This is the addition of $\reach(\avariable,\avariablebis) = 3$ that is crucial for undecidability since
the satisfiability problem for $\seplogic{\separate, \magicwand,\reach(\avariable,\avariablebis) = 2}$
is in \pspace~\cite{Demrietal17}.%%
%%
\OnlyForVL{\input{proof-corollary-undecidability-limited-reach}}%%
%%
%%
%% SD 15/10/2017
%%
%% I believe that the result holds but we need a refine our translation (because of
%% the current assumption that distinct quantifications should ue distinct variables.
%% We should speak about it in the long version but not here.
%%
\OnlyForVL{
Similarly, since $\foseplogic{\magicwand}$  restricted to two quantified variables
is undecidable~\cite{DemriDeters15}, we obtain the following result.

\begin{theorem}
The satisfiability problem for $\seplogic{\separate, \magicwand, \ls}$ restricted to four program
variables is undecidable.
\end{theorem}
}
Following a similar analysis, let SL1($\forall,\separate,\magicwand$) be the
restriction of $\foseplogic{\separate, \magicwand}$ (i.e.  $\foseplogic{\magicwand}$ plus separating conjunction $\separate$)
to formulae of the form
$
\exists \avariable_1 \ \cdots \  \exists \avariable_q \ \aformula
$,
where $q \geq 1$, the variables in $\aformula$ are among $\set{\avariable_1, \ldots, \avariable_{q+1}}$
and the only quantified variable in $\aformula$ is $\avariable_{q+1}$.
The satisfiability problem for SL1($\forall,\separate,\magicwand$) is \pspace-complete~\cite{Demrietal17}.
Note that SL1($\forall,\separate,\magicwand$) can easily express $n(\avariable) = n(\avariablebis)$
and $\allocback{\avariable}$.
The distance  between the decidability for SL1($\forall,\separate,\magicwand$)
and the undecidability for $\seplogic{\separate, \magicwand, \ls}$, is best witnessed by the corollary below,
which solves an open problem~\cite[Section 6]{Demrietal17}.%%
%%
\begin{corollary} SL1($\forall,\separate,\magicwand$) augmented with
$n(\avariable) \hpto n(\avariablebis)$ (resp. SL1($\forall,\separate,\magicwand$) augmented with $\ls$) admits an undecidable satisfiability problem.
\end{corollary}%%

